SpikeVLA: Vision-Language-Action Models with Spiking Neural Networks

Vision-Language-Action (VLA) models have become a dominant paradigm for embodied intelligence. However, most existing approaches are built on large-scale transformers, resulting in substantial inference latency and energy consumption that limit their practical deployment in low-power, real-time scenarios. We propose SpikeVLA, a spiking VLA architecture for embodied navigation with energy-efficient inference, consisting of three key components. (i) A spiking vision encoder, Spike-V, that replaces dense continuous layers with event-driven spiking layers to reduce the energy consumption of visual representation learning. (ii) A multi-modal spiking large language model, Spike-L, that reformulates cross-modal reasoning with spiking dynamics and token-level event-driven sparsity to further lower computational cost. (iii) A spiking action policy network, Spike-A employs Laplacian-kernel population coding with a multi-layer fully connected SNN, and decodes spiking activities into stable and robust continuous control with energy-efficient inference under low-power constraints. Experiments on navigation and robotic control tasks show that SpikeVLA significantly reduces energy consumption and computational cost while maintaining competitive performance, highlighting its potential for low-power, real-time embodied intelligence.

==> section/copy.tex <==
\section{Method}
\label{sec:method}

\subsection{Problem Formulation}
\subsection{Spike Neural Network Vision Encoder}
ANN-based visual encoders are widely used in robotic system due to their ability to extract rich features from visual frames. However, their high computational cost and energy consumption can be prohibitive, especially in resource-constrained environments. To overcome these challenges, we propose a spiking neural network-based vision encoder and provide a detailed description of its construction process in this section.

\noindent\textbf{Neuron Vision Encoder.}
The input to the model includes not only the current frame image but also incorporates historical frame images, which is essential for adapting to our VLA model. By fusing the current and historical frame information, the model is better able to capture dynamic changes in the temporal dimension, enhancing its understanding of visual tasks, particularly in scenarios with complex temporal dependencies. 
% We employ SigLip as the vision encoder, which effectively extracts temporal information between the current and historical frames, providing rich visual representations for subsequent tasks, thereby improving the model's performance in dynamic environments.
% \textbf{Objective:} This section will provide a detailed explanation of the theoretical conversion from ANN to SNN, demonstrating that under certain conditions, ANN can be converted to SNN while ensuring a feasible mapping between the two.

In traditional, the computation of neurons is realized through the combination of linear transformations and non-linear activation functions. However, the SNN is simulated over \( T \) time points, where the vector of membrane potentials of neurons at time \( t \), i.e., the post-synaptic potential released from layer \( l-1 \) to layer \( l \), is collected to model the source ANN. The forward process corresponding to the source ANN and the target SNN can be described as follows:
\begin{equation}
\mathbf{y}_{l}=A\left( \mathbf{W}_{l}\cdot \mathbf{y}_{l-1}\right),\quad 
\mathbf{\hat{y}}_{l} =S\left( \mathbf{W}_{l}\cdot \mathbf{\hat{y}}_{l-1} \right) 
\end{equation}
where $\mathbf{y}$ is the activation vector of the current layer, $\mathbf{W}_{l}$ is the weight matrix, and $\mathbf{A}(\cdot) $ and $\mathbf{S}(\cdot)$ are the ANN activation function and SNN activation function respectively.

In SNN, the activation mechanism of neurons is based on the accumulation of membrane potentials, which trigger spikes once the membrane potential reaches a certain threshold. Unlike traditional activation functions, SNN uses an Integrate-and-Fire (IF) model for computation.
\begin{equation}
\mathbf{v}^{\prime }_{l}(t)=\mathbf{v}_{l}(t-1)+\mathbf{W}_{l}\cdot \mathbf{x}_{l-1}(t)\cdot \mathbf{\theta}_{l-1} 
\end{equation}
\begin{equation}
\mathbf{x}_{l}(t)=\mathbf{G}(\mathbf{v}^{\prime }_{l}(t) - \theta_l)
\end{equation}
\begin{equation}
\mathbf{v}_l(t) = \mathbf{v}_{l}(t-1)+\mathbf{W}_{l}\cdot \mathbf{x}_{l-1}(t)\cdot \mathbf{\theta}_{l}  - \mathbf{x}_{l}(t)\cdot\theta_l
\end{equation}
where \(\mathbf{v}^{\prime }_{l}(t)\) is the membrane potential of the \(i\)-th neuron at time \(t\), \( \mathbf{W}_{l} \) is the weights from last layer.  \( \theta_l \) is the firing threshold, and \( \mathbf{G(\cdot)} \) is the Heaviside step function.



% \noindent\textbf{Proof of Conversion Feasibility}

% We aim to prove that the conversion from ANN to SNN is feasible. By mapping the activation functions from ANN to the spike emission mechanism of SNN, we obtain the following equation that demonstrates the relationship between the activation values in ANN and the membrane potential in SNN.

The activation values of ANN can be represented by the firing rate of the SNN. Assuming the initial membrane potential \( \mathbf{v}_l(0) \), and cumulating neuron functions from \( t = 1 \) to \( T \), the relationship between activation and SNN and rate can be expressed as:
\begin{equation}
\mathbf{v}_l(T) = \mathbf{v}_l(0) + \mathbf{W}_l \cdot \sum_{t=1}^{T} \mathbf{x}_{l-1}(t)\cdot \mathbf{\theta}_{l-1}  - \sum_{t=1}^{T} \mathbf{x}_l(t) \cdot \theta_l(t)
\end{equation}
This expression reveals the linear relationship between the activation values in ANN and the firing rate in SNN. By defining the average post-synaptic potential \( \mathbf{\hat{y}}_{l} \) as:
\begin{equation}
\mathbf{\hat{y}}_{l}(t)=\frac{\sum^{T}_{t=1} \mathbf{x}_{l} (t)\cdot \theta_{l} (t)}{t} 
\end{equation}
we can reformulate the above equation as:
\begin{equation}
\begin{split}
\mathbf{\hat{y}}_{l} (T)=\frac{\mathbf{W}_{l}} {T} \cdot \sum^{T}_{t=1} \mathbf{x}_{l-1} (t)\cdot \mathbf{\theta }_{l-1} -\frac{\mathbf{v}_{l}(T)-\mathbf{v}_{l}(0)}{T}
\end{split}
\end{equation}
% \begin{align}
% \mathbf{\hat{y}}_{l} (T) &= \frac{\mathbf{W}_{l}}{T} \cdot \sum_{t=1}^{T} \mathbf{x}_{l-1} (t) \cdot \mathbf{\theta }_{l-1} - \frac{\mathbf{v}_{l}(T) - \mathbf{v}_{l}(0)}{T} \\
% &= \mathbf{W}_{l} \cdot \mathbf{\hat{y}}_{l-1} (t) - \frac{\mathbf{v}_{l}(T) - \mathbf{v}_{l}(0)}{T}
% \end{align}
As \( T\to+\infty \), the equations can be further simplified as follows: 
\begin{equation}
\begin{aligned}
\mathbf{\hat{y}}_{l} (T) &= \mathbf{W}_{l} \cdot \mathbf{\hat{y}}_{l-1}  (t) - \frac{\mathbf{v}_{l}(T) - \mathbf{v}_{l}(0)}{T} \\
 &:= S\left( \mathbf{W}_{l} \cdot \mathbf{\hat{y}}_{l-1}  (t) \right)
\end{aligned}
\end{equation}


Therefore, by replacing the neuron activation functions with Integrate-and-Fire (IF) neurons, the ANN model can be approximately converted into an SNN using the presented equations.

\noindent\textbf{Objective Function Definition.} We aim to minimize the error between ANN and SNN during the conversion process. The conversion error \( \epsilon^{(l)} \) is defined as the difference between the post-synaptic potential in SNN and the activation output in ANN:
\begin{equation}
\Delta \mathcal{L} = \left\| S(\mathbf{\hat{y}}_{l},  \theta_{l}) - A(y_{l}) \right\|^2
\end{equation}
where \( \mathbf{\hat{y}}_{l} = \mathbf{W}_{l} \cdot \mathbf{\hat{y}}_{l-1} \) is the input to SNN, \( A(\cdot) \) is the activation output in ANN, \( S(\cdot) \) is the spike response in SNN, and \( \epsilon_{l} \) is the conversion error.

To optimize the objective function, we adjust the weights and thresholds to minimize the error and ensure that SNN correctly simulates the behavior of ANN. To further optimize the error, we derive an upper bound for the error:
\begin{equation}
\Delta \mathcal{L}_l \leq \left\| S(\mathbf{\hat{y}}_{l},  \theta_{l}) - A(y_{l}) \right\|^2 + C\left\| \mathbf{W}_{l} \right\|^2 \Delta \mathcal{L}_{l-1}
\end{equation}

By adjusting the weights and thresholds for each layer, we can reduce the accumulation of error and ensure the accuracy of the SNN.
The objective is to minimize the error between SNN and ANN during the conversion. The specific objective function is defined as:

\begin{equation}
\arg \min_{\theta} \mathbb{E}_{x_0 \in D} \left[ \sum_{l=1}^{L} \prod_{k=l+1}^{L} C\| \mathbf{W}_k \|_2 \left\| S(\mathbf{\hat{y}}_{l},  \theta_{l}) - A(y_{l}) \right\|^2 \right]
\end{equation}

where \( \theta = \{ \theta_1, \theta_2, \dots, \theta_L \} \) represents the thresholds for each layer, \( x_0 \) is a sample drawn from the dataset \( D \), and \( S(\hat{z}^{(l)}; \theta^{(l)}) \) is the output of the SNN, \( A(\hat{z}^{(l)}) \) is the activation output in ANN.

We use the squared norm for optimization, which transforms the optimization process into:

\[
\arg \min_{\theta_l} \mathbb{E}_{x_0 \in D} \left[ \prod_{k=l+1}^{L} \| \mathbf{W}_k \|_2 \left| C(\hat{z}^{(l)}; \theta^{(l)}) - A(\hat{z}^{(l)}) \right|_2^2 \right]
\]

where the clipping function \( C(x; \theta) \) is defined as:

\[
C(x; \theta) = \min(\max(0, x), \theta)
\]

During the optimization process, we use **stochastic gradient descent (SGD)** to update the thresholds \( \theta^{(l)} \) for each layer. The update rule is as follows:

\[
\Delta \theta^{(l)} = - \sum_{i=0}^{N-1} 2(\hat{z}^{(l)}_i - \theta^{(l)}) \mathbb{H}(\hat{z}^{(l)}_i - \theta^{(l)})
\]
\[
\theta^{(l)} \leftarrow \theta^{(l)} - \eta \Delta \theta^{(l)}
\]

where \( \Delta \theta^{(l)} \) is the update step for each layer, \( \eta \) is the learning rate, \( N \) is the number of elements in the input vector, \( \hat{z}^{(l)}_i \) is the \( i \)-th element of the input vector, and \( \mathbb{H}(\cdot) \) is the Heaviside step function.



By combining techniques such as local threshold balancing, weight scaling, pooling layer replacement, and activation function adjustment, the proposed Spike Neural Network Vision Encoder efficiently retains the visual encoding capability while optimizing energy efficiency, ensuring high-performance inference in low-power environments. The event-driven of spiking neurons, which enable computationally efficient processing, also preserve high accuracy in complex and dynamic environments.


\subsection{Multimodal Spiking Large Language Model}

We present SpikeVLM, which unifies visual and textual inputs into a single token stream and processes them with a spiking vision language model. We adopt a Generalized Integrate-and-Fire spiking mechanism to encode visual and text tokens, which produces temporally sparse representations. (ii) We propose a channel-saliency metric that exploits Fisher/Hessian-based second-order sensitivity and temporal characteristics of visual and text token representations to allocate longer spike steps to informative channels, which enables more compute- and energy-efficient inference.

\noindent\textbf{Unified Token Representations.}
We map history frames, current frame, and text into a shared latent space and concatenate them into a unified sequence.
\begin{equation}
\mathcal{S}_0 \;=\; \big[\,\mathbf{V}^{\mathrm{hist}},\ \mathbf{V}^{\mathrm{cur}},\ \mathbf{T}\,\big]
\in \mathbb{R}^{(196t + 196 + N_{\mathrm{text}})\times d},
\end{equation}
where $\mathbf{V}^{\mathrm{hist}} \in \mathbb{R}^{(196\cdot t)\times d}$ are history visual tokens, $\mathbf{V}^{\mathrm{cur}} \in \mathbb{R}^{196\times d}$ are current visual tokens, $\mathbf{T} \in \mathbb{R}^{N_{\mathrm{text}}\times d}$ are text tokens, $d$ is the shared hidden size, and $t$ is the number of history frames. 

\noindent\textbf{Spiking Dynamics on Unified Tokens.}
To convert the unified token representations into sparse spike tokens, we evolve each token under spiking neuron dynamics and merge fine time steps.
Each token receives a projected input and evolves under with spike dynamics at fine time steps $u$:
\begin{equation}
\begin{aligned}
\tilde V_{i,u} &= \alpha\, V_{i,u-1} + (\mathcal{S}_{0,i} W_{\mathrm{in}} + b) - \beta\, S_{i,u-1},\\
S_{i,u} &= \mathbf{1}\!\big(\tilde V_{i,u} \ge \vartheta\big), \quad
V_{i,u} = \tilde V_{i,u} - \vartheta\, S_{i,u}.
\end{aligned}
\end{equation}
where $\mathcal{S}_{0,i}$ is the $i$-th token, $W_{\mathrm{in}},b$ are input projection parameters, $V_{i,u}$ is the membrane potential, $S_{i,u}\!\in\!\{0,1\}$ is the spike, $\alpha\!\in\!(0,1)$ is the leak, $\beta\!\ge\!0$ models after-spike hyperpolarization, and $\vartheta$ is the threshold. To stabilize training and shorten the effective horizon, we merge $L$ consecutive fine steps into a multi-level spike:
\begin{equation}
s_i[t']=\sum_{u=t'L}^{(t'+1)L-1} S_{i,u},\quad
t'=0,\ldots,T'-1,\ \ T'=\tfrac{T}{L}.
\end{equation}
where $L$ denotes the merge window, $T$ and $T'$ denote the numbers of fine-grained time steps before and after merging, respectively, and $s_i(t')\in\{0,\ldots,L\}$ is the spike count.

\noindent\textbf{Differential Temporal Sparsity Allocation.}
To evaluate the importance of channels across different modalities and within the same modality, we propose a differential temporal sparsity allocation mechanism. More specifically, we give longer steps to more informative channels and one-step spikes to less significant ones. This process is formalized as follows for a single modality:
\begin{equation}
{h}^{(k)} = \frac{V_{\text{max}}}{L'} \sum_{t=1}^{L'} p^{(k)}_t + \min({h}^{(k-1)}),
\end{equation}
where \({h}^{(k)}\) represents the saliency score of the \( k \)-th channel at the current step, \( V_{\text{max}} \) is the per-token spiking threshold, controlling the firing threshold for spikes. \( L' \) is the number of steps, \( p^{(k)}_t \) is the spiking activity of the \( k \)-th channel at time step \( t \), and \( \min({h}^{(k-1)}) \) ensures smooth transition of the saliency score.

Considering the importance metric across different modalities, we extend the channel computation to a multimodal scenario, as expressed in the following formula:
\begin{equation}
\tilde{h}^{(k)} = \frac{V_{\text{max}}}{L'} \sum_{t=1}^{L'} p^{(k)}_t \Big|_{p \in S_{\text{mod}}} + \min(\tilde{h}^{(k-1)}),
\end{equation}
where \( S_{\text{mod}} \) is the set of all channels within the current modality (e.g., visual or text), and \( S_m \) is the set of significant channels in each modality \( m \in \mathcal{M} \). 

Next, we further extend this formula to allocate longer spiking steps to significant channels within each modality and consider cross-modal significance. The extended formula, incorporating both within-modality and cross-modality channel importance, is given by:
\begin{equation}
\begin{split}
\tilde{x}^{(k)} \approx & \frac{V_{\text{max}}}{L'} \sum_{t=1}^{L'} p^{(k)}_t \Big|_{p \in S_{\text{imp}}} + s^{(k)}(1) \cdot V_{\text{max}} \Big|_{p \in  S_{\text{mod}}} \\
&+ \min(\tilde{x}^{(k-1)}),
\end{split}
\end{equation}
where \( S_{\text{imp}} \) represents the set of significant channels in the current modality, \( S_{\text{mod}} \) is the set of all channels within the current modality, and \( s^{(k)}(1) \) is the initial spike activity of the \( k \)-th channel. This extension allows for more detailed saliency weighting based on modality and channel importance.

This framework unifies vision and language into a single spiking token stream by using spike coding and step allocation guided by channel importance, which directs computation toward essential information.
This approach selectively allocates spiking steps based on the importance of channels both across and within modalities, which ensures efficient computation and energy savings.



\subsection{Spiking Neural Network for Action Policy}
We propose an action policy network based on Spiking Neural Networks (SNNs). The input is converted into spikes through Fourier encoding and processed by multiple fully connected SNN layers, during which the neurons' currents, membrane potentials, and spikes are continuously updated. The final action is generated through a decoding module. During reinforcement learning, the network is trained using the Proximal Policy Optimization (PPO) algorithm to optimize its parameters.

\noindent\textbf{Fourier Encoding and Decoding Network.}
To encode the observation values into the activity of neuron populations, Fourier encoding is used to compute the activity of the population of neurons. Fourier encoding maps each observation dimension \( s_i \) (\( i \in \{1, 2, \dots, N\} \)) into a high-dimensional periodic space using sine and cosine functions. The encoding is given by the following formula:
\begin{equation}
\begin{aligned}
A_E = \Big[ &\sin(2 \pi f_1 s_i), \cos(2 \pi f_1 s_i), \dots \\
           &\sin(2 \pi f_k s_i), \cos(2 \pi f_k s_i) \Big]
\end{aligned}
\end{equation}
where \( f_1, \dots, f_k \) are predefined frequency parameters, and \( s_i \) is the \( i \)-th dimension of the observation. Fourier encoding offers the advantage of efficiently capturing complex input patterns and global features, especially for data with periodic characteristics. 

The resulting activity \( A_E \) is used as the stimulus for the neuron populations, which then propagate through the SNN to generate spikes. 
We use a deterministic encoding scheme, where the membrane potential of the neurons is updated according to the following equation:
\begin{equation}
z_l(t) = \alpha_l \cdot z_{l-1}(t) + W_l \cdot a_{l-1}(t) + b_l
\end{equation}
\begin{equation}
u_l(t) = \beta_l \cdot u_{l-1}(t) \cdot (1 - a_{l-1}(t)) + z_l(t)
\end{equation}
\begin{equation}
a_l(t) = \text{Activation}(u_l(t))
\end{equation}
Where \( z_l(t) \) is the current at time step \( t \) for layer \( l \). \( u_l(t) \) is the membrane potential for layer \( l \). The spike output \( a_l(t) \) is generated by applying an activation function to \( u_l(t) \). \( \alpha_l \) and \( \beta_l \) are decay factors for current and membrane potential, and \( W_l \) is the weight matrix for layer \( l \).

In the decoding module, the total spike count for each action dimension is accumulated over \(T\) time steps, and the firing rate \(fr(i)\) is computed as the average spike count per time step. The final action \(a_i\) for each output dimension is then generated by applying the learned decoding weight and bias. The full expression is as follows:
\begin{equation}
a_i = W_d^{(i)} \cdot \frac{1}{T} \sum_{t=1}^{T} o^{(K)}_i(t) + b_d^{(i)}
\end{equation}
Where \( a_i \) is the action for the \( i \)-th output dimension, \( W_d^{(i)} \) is the decoding weight for the \( i \)-th action dimension. \( o^{(K)}_i(t) \) represents the spike from the \( i \)-th output neuron in layer \( K \) at time step \( t \). 



\noindent\textbf{Reinforcement Learning Training.}
In the training phase, we optimize the SNN using the PPO (Proximal Policy Optimization) algorithm. PPO trains the network by optimizing the clipped surrogate loss, aiming to improve the mean of the action distribution. During training, the network generates actions based on observed states and adjusts its policy using feedback from the critic network.

The policy ratio \( r_t(\theta) \) is the ratio of the action probabilities under the current policy \( \pi_\theta \) to those under the old policy \( \pi_{\theta_{\text{old}}} \), given by:
\begin{equation}
r_t(\theta) = \frac{\pi_\theta(a_t | s_t)}{\pi_{\theta_{\text{old}}}(a_t | s_t)}
\end{equation}
Where \( a_t \) is the action taken at time step \( t \).
\( s_t \) is the observed state at time step \( t \).

The advantage function \( \hat{A}_t \), computed by the critic network, indicates how much better the action \( a_t \) is compared to the baseline. It is given by:
\begin{equation}
\hat{A}_t = Q(s_t, a_t) - V(s_t)
\end{equation}
Where \( Q(s_t, a_t) \) is the action-value function, which represents the expected return from taking action \( a_t \) in state \( s_t \).
- \( V(s_t) \) is the state-value function, which represents the expected return from state \( s_t \).

The PPO objective is optimized using the surrogate loss function. This function balances maximizing the expected return with preventing excessively large updates by clipping the policy ratio. The PPO loss function is defined as:
\begin{equation}
L^{\text{PPO}}(\theta) = \mathbb{E}_t \left[ \min \left( r_t(\theta) \hat{A}_t, \text{clip}(r_t(\theta), 1 - \epsilon, 1 + \epsilon) \hat{A}_t \right) \right]
\end{equation}
Here, the clip function ensures that the policy update is bounded, preventing large deviations from the previous policy, which enhances stability.

For continuous action spaces, the action \( a_t \) is predicted by the actor network as the mean \( \mu_t \) and standard deviation \( \sigma_t \) of a Gaussian distribution.
This allows the network to generate actions that are drawn from a continuous distribution, suitable for fine-grained control.

PPO trains the SNN action network by optimizing the surrogate loss function. The actor network generates actions based on the observed state, while the critic network estimates their value. The clipped surrogate loss ensures stable policy updates. Network parameters are updated using the PPO loss gradients, achieving an optimal policy that balances exploration and exploitation in continuous action spaces.

% The parameters of the SNN are updated using gradient descent. Specifically, for the output layer parameters \( W_i \) and \( b_i \) (\( i \in \{1, 2, \dots, M\} \)), the update rule is:
% \begin{equation}
% \nabla W_i L = \nabla a_i L \cdot W_i \cdot fr_i, \quad \nabla b_i L = \nabla a_i L \cdot W_i
% \end{equation}
% where \( \nabla a_i L \) is the gradient of the loss function \( L \) with respect to action \( a_i \), \( fr_i \) is the firing rate of population \( i \), and \( W_i \) is the connection weight.

% SNN parameters (weights and biases) are updated using spatiotemporal backpropagation. For each layer \( k \), the gradients are computed by accumulating over time steps \( T \) as follows:
% \begin{equation}
% \nabla W_k L = \sum_{t=1}^T o(t)^{(k-1)} \cdot \nabla c(t)^{(k)} L, 
% \end{equation}
% \begin{equation}
% \quad \nabla b_k L = \sum_{t=1}^T \nabla c(t)^{(k)} L
% \end{equation}
% where \( o(t)^{(k-1)} \) represents the spikes from the previous layer, and \( \nabla c(t)^{(k)} L \) is the gradient of the loss function \( L \) with respect to the current layer's current \( c(t)^{(k)} \).

% For the input populations \( i \) (\( i \in \{1, 2, \dots, N\} \)), the update rule for encoding parameters (such as \( \mu_i \) and \( \sigma_i \)) is as follows:
% \begin{equation}
% \nabla \mu_i L = \sum_{t=1}^T \nabla o(t)(0)_i L \cdot A_E(i) \cdot \frac{s_i - \mu_i}{\sigma_i^2}, 
% \end{equation}
% \begin{equation}
% \quad \nabla \sigma_i L = \sum_{t=1}^T \nabla o(t)(0)_i L \cdot A_E(i) \cdot \frac{(s_i - \mu_i)^2}{\sigma_i^3}
% \end{equation}
% where \( \nabla o(t)(0)_i L \) is the gradient of the loss function \( L \) with respect to the input \( s_i \), \( A_E(i) \) is the output of the Fourier encoding, and \( \mu_i \) and \( \sigma_i \) are the mean and standard deviation of the input population.

% Every \( T \) time steps, all parameters are updated using these gradients. Through spatiotemporal backpropagation, gradients are propagated from the output layer to the input layer, ensuring that the weights and biases of each neuron population are updated appropriately.

% \( W_i \) and \( b_i \): The weights and biases of output population \( i \), controlling the strength of neuron connections and activation.
% \( a_i \): The action produced by output population \( i \), representing the decision made by the network.
% \( fr_i \): The firing rate of population \( i \), i.e., the average spike rate of the neurons in that population.
% \( o(t)^{(k-1)} \): The spike output of neurons from layer \( k-1 \) at time step \( t \).
% \( c(t)^{(k)} \): The current of neurons in layer \( k \) at time step \( t \).
% \( \nabla c(t)^{(k)} L \): The gradient of the loss function \( L \) with respect to current \( c(t)^{(k)} \).
% \( \mu_i \) and \( \sigma_i \): The mean and standard deviation of input population \( i \), which control the Fourier encoding process.









==> tables/ablation_action.tex <==
\begin{table}[!t]
\centering
\caption{Ablation study on hyperparameters of the action policy. The baseline configuration is marked with $\ast$. Results evaluate tracking accuracy and resource efficiency.}
\label{tab:action_ablation}
\renewcommand{\arraystretch}{1} % 增加行高，更显优雅
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{llccccc}
\toprule
\multirow{2}{*}{\textbf{Category}} & \multirow{2}{*}{\textbf{Configuration}} & \multicolumn{2}{c}{\textbf{Tracking Error}} & \multicolumn{3}{c}{\textbf{Resource Efficiency} } \\
\cmidrule(lr){3-4} \cmidrule(lr){5-7}
& & Linear Vel.$\downarrow$ & Angular Vel.$\downarrow$ & Mem(MB)$\downarrow$ & Eng(\textmu J)$\downarrow$ & ACEs($10^{6}$)$\downarrow$ \\
\midrule
% --- T 的消融 ---
\multirow{3}{*}{Time Step ($T$)} 
& $T=2$ & 0.44 & 0.55 & 2.35 & 0.07 &1.24\\
& $T=3^\ast$ & 0.35 & 0.47 & 2.35 & 0.10 &1.76\\
& $T=5$ & 0.35 & 0.45 & 2.35 & 0.31 &5.53\\
\midrule
% --- Popdim 的消融 ---
\multirow{3}{*}{Pop. Dim ($P$)} 
& $P=2$ & 0.77 & 0.59 & 0.98 & 0.03&0.53 \\
& $P=3$ & 0.65 & 0.68 & 1.43 & 0.15 & 2.62 \\
& $P=5^\ast$ & 0.35 & 0.47 & 2.35 & 0.10 & 1.76 \\
\midrule
% --- Actor 的消融 ---
\multirow{3}{*}{Actor Arch.} 
& [128, 128]$^\ast$ & 0.35& 0.47 & 2.35 & 0.10 &1.76 \\
& [256, 128] & 0.43 & 0.48 & 4.63 & 0.17 & 2.96 \\
& [256, 256] & 0.34 & 0.49 & 4.48 & 0.34 & 6.14 \\
\midrule
% --- Critic 的消融 ---
\multirow{3}{*}{Critic Arch.} 
& [512, 256, 128]$^\ast$ & 0.35 & 0.47 & 2.35 & 0.10 &1.76 \\
& [512, 256, 256] & 0.49 & 0.54 & 2.35 & 0.09 & 1.58\\
& [256, 256, 128] & 0.44 & 0.51 & 2.35 & 0.15 & 2.72\\
\bottomrule
\end{tabular}}
\end{table}

==> tables/benchmark.tex <==
\begin{table*}[!t]
\centering
\small
\setlength{\tabcolsep}{2pt}
\caption{VLN-CE-Isaac evaluation results.}
\vspace{-0.5em}
\scalebox{0.97}{
{\fontsize{8pt}{9pt}\selectfont
\begin{tabular}{lcccccccccc}
\toprule
& \multicolumn{3}{c}{Low-level Observation} &  \multicolumn{4}{c|}{VLN-CE-Isaac} & \multicolumn{3}{c|}{Computational Cost}\\
\cmidrule(lr){2-4} \cmidrule(lr){5-8} \cmidrule(lr){9-11}
& Proprio. & LiDAR & Height Scan & NE $\downarrow$ & OS $\uparrow$ & SR $\uparrow$ & SPL $\uparrow$ & T $\downarrow$ & M $\downarrow$ & E $\downarrow$ \\
\midrule
\textit{Oracle} & & &   & \textit{5.25} & \textit{59.8} & \textit{51.3} & \textit{46.9} & & &\\
\midrule
\multicolumn{11}{l}{\bf\emph{Unitree Go2}} \\
% NaVILA-Blind* & \checkmark & & &  6.03* & 49.0* & 36.2* & 33.3* & & &\\
% NaVILA-Blind(reproduce) & \checkmark & & &  &  &  &  & & &\\
% NaVILA-Vision* & \checkmark & \checkmark & &  \textbf{5.49*} & \textbf{58.7*} & \textbf{50.2*} &  \textbf{45.5*}& & &\\
% NaVILA-Vision(reproduce) & \checkmark & & &  3.63 & 57.7 & 44.8 & 41.9 & & &\\

SpikeVLA-Blind & \checkmark & &    & 4.27 & 48.8 & 33.1 &29.2 && &\\
SpikeVLA-Vision & \checkmark & \checkmark & &   &  &  &  & & &\\
% \midrule
% \multicolumn{11}{l}{\bf\emph{Unitree H1}} \\
% NaVILA-Blind & \checkmark & &  &  7.67* & 33.3* & 24.4* & 21.0*& & &\\
% NaVILA-Vision & \checkmark & & \checkmark &  \textbf{5.86*}& \textbf{54.6*} & \textbf{45.3*} & \textbf{40.3*} & & &\\
\bottomrule
\end{tabular}}}
\vspace{-5pt}
\label{tab:r2r_isaac}
\end{table*}

==> tables/quant.tex <==
\begin{table}[!t]
\centering
\small
\setlength{\tabcolsep}{2pt}
\caption{quant effect L20}
\vspace{-0.5em}
\scalebox{0.97}{
{\fontsize{8pt}{9pt}\selectfont
\begin{tabular}{lcc}
\toprule
quant method & inference speed (token/s) &  memory usage (MB) \\
\midrule
no quantization& 43.63 & 20817.61\\
SpikeLLM & 126.7 & 5824.43\\
OmniQuant & 127.6 & 5897.89\\

\bottomrule
\end{tabular}}}
\vspace{-5pt}
\label{tab:quant}
\end{table}

==> tables/siglip.tex <==
% ---------- Table A1: Operator replacement summary (camera-ready) ----------
\begin{table}[t]
\centering
\caption{Detailed Architecture of the Spiking Visual Encoder.}
\small
\renewcommand{\arraystretch}{1.12}
\setlength{\tabcolsep}{5.5pt}
\begin{tabular}{l l l l}
\toprule
\textbf{Component} & \textbf{ANN Layer} & \textbf{SNN Layer} & \textbf{Purpose} \\
\midrule
% Patch embedding
% & Conv2d
% & \texttt{MTH\_diff\_line} + Conv2d
% & Spiking gating for patch tokens. \\

% Positional encoding
% & Embedding
% & Embedding
% & Preserve token positions. \\

Q/K/V projections
& Linear
& Spike Linear 
& Spiking-aware temporal projections. \\

Normalization
& LayerNorm
& SpikeLN
& Stable multi-step normalization. \\

MLP nonlinearity
& GELU/Tanh
& SpikeGELU/SpikeTanh
& Spike-compatible nonlinearity. \\

Attention softmax
& Softmax
& SpikeSoftmax
& Stable attention normalization. \\

% Attention modulation
% & --
% & \texttt{AtNeuron} (+ \texttt{MyatSequential})
% & Event-driven attention. \\

Pooling head
& Attn Pool + MLP
& Attn Pool + \texttt{exp\_comp\_neuron}(LN/MLP)
& Spiking-wrapped pooling head. \\
\bottomrule
\end{tabular}
\label{tab:spike_siglipv2_ops}
\vspace{-2mm}
\end{table}


==> tables/vlm.tex <==
\begin{table*}[t]
    \small
    \centering
    \caption{Comparison with state-of-the-art methods on the Val-Unseen split of R2R-CE~\citep{r2r} and RxR-CE~\citep{rxr}. $^{*}$ indicates methods using the waypoint predictor from~\citet{hong2022bridging}. we outperforms all methods that do not rely on simulator pre-trained waypoint predictors, even when those methods leverage additional inputs such as depth, panoramic views, and odometry.}
    % \vspace{-5pt}
    \setlength{\tabcolsep}{7.0pt}
    \scalebox{0.85}{
{\fontsize{8pt}{9pt}\selectfont
\begin{tabular}{l|cccc|lcccclccccccc}
\toprule
& \multicolumn{4}{c}{Observation} &  \multicolumn{4}{c}{R2R Val-Unseen}  & \multicolumn{4}{c}{RxR Val-Unseen} & \multicolumn{3}{c}{Computational Cost}\\
\cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} \cmidrule(lr){14-16}
& S.RGB & Pano. & Depth & Odo. & NE $\downarrow$ & OS $\uparrow$ & SR $\uparrow$ & SPL $\uparrow$ & NE $\downarrow$ & SR $\uparrow$ & SPL $\uparrow$ & nDTW $\uparrow$ & T $\downarrow$ & M $\downarrow$ & E $\downarrow$\\
\midrule
HPN+DN$^{*}$~\citep{krantz2021waypoint}   & \checkmark & \checkmark & \checkmark  && 6.31 & 40.0 & 36.0 & 34.0  & - & - & - & - &&&\\
CMA$^{*}$~\citep{hong2022bridging}  & \checkmark & \checkmark & \checkmark && 6.20 & 52.0 & 41.0 & 36.0  & 8.76 & 26.5 & 22.1 & 47.0 &&&\\
VLN$\circlearrowright$BERT$^{*}$~\citep{hong2022bridging}  & \checkmark & \checkmark & \checkmark & & 5.74 & 53.0 & 44.0 & 39.0  & 8.98 & 27.0 & 22.6 & 46.7 &&&\\
Sim2Sim$^{*}$~\citep{krantz2022sim}  & \checkmark  & \checkmark & \checkmark  && 6.07 & 52.0 & 43.0 & 36.0 & - & - & - & - &&&\\
GridMM$^{*}$~\citep{wang2023gridmm}  & \checkmark  & \checkmark & \checkmark  && 5.11 & 61.0 & 49.0 & 41.0  & - & - & - & - &&&\\
Ego$^{2}$-Map$^{*}$~\citep{hong2023learning}  & \checkmark  & \checkmark & \checkmark & & 5.54 & 56.0 & 47.0 & 41.0  & - & - & - & - &&&\\
DreamWalker$^{*}$~\citep{wang2023dreamwalker}  & \checkmark  & \checkmark & \checkmark & & 5.53 & 59.0 & 49.0 & 44.0  & - & - & - & - &&&\\
Reborn$^{*}$~\citep{an20221st}  & \checkmark  & \checkmark & \checkmark & & 5.40 & 57.0 & 50.0 & 46.0 & 5.98 & 48.6 & 42.0 & 63.3 &&&\\
ETPNav$^{*}$~\citep{an2024etpnav}  & \checkmark  & \checkmark & \checkmark & & 4.71 & 65.0 & 57.0 & 49.0 & 5.64 & 54.7 & 44.8 & 61.9 &&&\\
HNR$^{*}$~\citep{wang2024lookahead}  & \checkmark  & \checkmark & \checkmark & & 4.42 & 67.0 & 61.0 & 51.0  & 5.50 & 56.3 & 46.7 & 63.5 &&&\\
BEVBert$^{*}$~\citep{an2023bevbert}  & \checkmark  & \checkmark & \checkmark & & 4.57 & 67.0 & 59.0 & 50.0  & 4.00 & 68.5 & - & 69.6 &&&\\
HAMT+ScaleVLN$^{*}$~\citep{wang2023scaling}  & \checkmark  & \checkmark & \checkmark & & 4.80 & - & 55.0 & 51.0  & - & - & - & - &&&\\
\midrule
AG-CMTP~\citep{chen2021topological}  & \checkmark  & \checkmark & \checkmark & & 7.90 & 39.0 & 23.0 & 19.0  & - & - & - & - &&&\\
R2R-CMTP~\citep{chen2021topological}  & \checkmark  & \checkmark & \checkmark & & 7.90 & 38.0 & 26.0 & 22.0  & - & - & - & - &&&\\
LAW~\citep{raychaudhuri2021language} & \checkmark  & \checkmark & \checkmark & & 6.83 & 44.0 & 35.0 & 31.0  & 10.90 & 8.0 & 8.0 & 38.0 &&&\\
CM2~\citep{georgakis2022cross} & \checkmark  & \checkmark & \checkmark & & 7.02 & 41.0 & 34.0 & 27.0  & - & - & - & - &&&\\
WS-MGMap~\citep{chen2022weakly} & \checkmark  & \checkmark & \checkmark & & 6.28 & 47.0 & 38.0 & 34.0  & - & - & - & - &&&\\
AO-Planner~\citep{chen2024affordances}  & \checkmark & \checkmark & & & 5.55 & 59.0 & 47.0 & 33.0  & 7.06 & 43.3 & 30.5 & 50.1 &&&\\
Seq2Seq~\citep{krantz2020beyond} & \checkmark  & \checkmark & & & 7.77 & 37.0 & 25.0 & 22.0  & 12.10 & 13.9 & 11.9 & 30.8 &&&\\
CMA~\citep{krantz2020beyond} & \checkmark  & \checkmark & & & 7.37 & 40.0 & 32.0 & 30.0  & - & - & - & - &&&\\
RGB-Seq2Seq~\citep{krantz2020beyond} & \checkmark  & & & & 10.10 & 8.0 & 0.0 & 0.0  & - & - & - & - &&&\\
RGB-CMA~\citep{krantz2020beyond} & \checkmark  & & & &  9.55 & 10.0 & 5.0 & 4.0  & - & - & - & - &&&\\
NaVid~\citep{zhang2024navid} & \checkmark  & & & &  5.47 & 49.0 & 37.0 & 35.0  & - & - & - & - &&&\\
MapNav& \checkmark &  & & &  4.93 & 53.0 & 39.7 & 37.2  & - & - & - & - &&&\\
NaVILA & \checkmark   & & & & \bf5.22 & \bf62.5 & \bf54.0 & \bf49.0  & \bf6.77 & \bf49.3 & \bf44.0 & \bf58.8 &&&\\
UniNaVid& \checkmark  & & & &  5.58 & 53.3 & 47.0 & 42.7  & 6.24 &48.7 &40.9& - &&&\\
SpikeVLA-spikellm & \checkmark &&&&5.56&61.61&52.80&47.69\\
SpikeVLA-omniquant & \checkmark &&&&5.48&62.04&53.18&48.08\\
SpikeVLA-spikellm+encoder-snn & \checkmark &&&&&&&\\
SpikeVLA-omniquant+encoder-snn & \checkmark &&&&&&&\\
\bottomrule
\end{tabular}}}
\vspace{-15pt}
\label{tab:vlm}
\end{table*}


==> temp.tex <==
**ICML-style figure prompt (for a text-to-image / plotting assistant)**

Use the following detailed English prompt to generate the publication‑quality figure:

---

Title:  
**“Comparison of Static Memory, Energy, and ACEs for NaVILA and SpikeVLA across Vision Encoder, LLM, and Action Policy”**

Overall style and layout:  
- Clean, minimal, ICML‑style scientific figure suitable for a top AI conference paper.  
- Vector‑style graphics, smooth lines, no 3D effects, no gradients, no shadows.  
- Consistent sans‑serif font for all text (e.g., Helvetica/Arial).  
- Use a white background, high contrast, and color‑blind‑friendly palette (e.g., blue vs. orange).  
- The figure is horizontally split into two main panels:  
  - **Left panel:** grouped bar charts (NaVILA vs. SpikeVLA).  
  - **Right panel:** 6 pie charts (3 rows × 2 columns).

---

### Left Panel: Grouped bar charts for V, L, A

Goal: Show how **SpikeVLA** outperforms **NaVILA** on **Static Memory**, **Energy**, and **ACEs** in each of the three modules: Vision encoder (V), LLM (L), and Action policy (A), while respecting linear scales (no log scales). A is extremely small and should be highlighted with a magnified inset.

Data (per module, per model):

- **Static Memory**
  - NaVILA‑V: 808.93 MB  
  - NaVILA‑L: 15316.05 MB  
  - NaVILA‑A: 1.20 MB  
  - SpikeVLA‑V: 809.88 MB  
  - SpikeVLA‑L: 5439.30 MB  
  - SpikeVLA‑A: 2.35 MB  

- **Energy**
  - NaVILA‑V: 22.70 J  
  - NaVILA‑L: 118.55 J  
  - NaVILA‑A: 5.80 μJ (microjoules)  
  - SpikeVLA‑V: 6.29 J  
  - SpikeVLA‑L: 37.94 J  
  - SpikeVLA‑A: 0.31 μJ  

- **ACEs**
  - NaVILA‑V: 631.52 T (10¹²)  
  - NaVILA‑L: 3298.69 T  
  - NaVILA‑A: 161.48 M (10⁶)  
  - SpikeVLA‑V: 111.75 T  
  - SpikeVLA‑L: 997.86 T  
  - SpikeVLA‑A: 5.53 M  

Plotting requirements:

1. **Structure**
   - Three side‑by‑side grouped bar charts, all aligned vertically and sharing the same x‑axis categories (V, L, A):  
     - Left: Static Memory [MB]  
     - Middle: Energy [J, μJ]  
     - Right: ACEs [T, M]  
   - For each group (V, L, A), draw two bars:  
     - NaVILA (e.g., blue)  
     - SpikeVLA (e.g., orange)  
   - Keep **linear scales** on all axes; do not use log scales.

2. **Axes & labels**
   - X‑axis: three categories labeled **V**, **L**, **A** under each bar group.  
   - Y‑axes:
     - First chart: label “Static Memory (MB)”.  
     - Second chart: label “Energy”, with clear indication of units: “J” for V and L entries, and “μJ” for A in the legend or annotation.  
     - Third chart: label “ACEs”, with units clearly explained: “T = 10¹², M = 10⁶”.  
   - Tick labels should be readable but not cluttered; use numerical ticks that make comparison intuitive.

3. **Visual encoding**
   - Use **NaVILA** and **SpikeVLA** as the only legend entries; do not separate V/L/A in the legend (they are already on the x‑axis).  
   - Use the same color per model across all three bar charts; only height of bars changes.  
   - Ensure that differences between NaVILA and SpikeVLA are clearly visible in the L and V modules, even with linear axes.

4. **A‑module magnification (zoomed inset)**
   - Since **A** values are extremely small compared to V and L, keep the global axis linear but:  
     - In each of the three bar charts, indicate the A bars with a small rectangle/frame or “cut‑out” region.  
     - From each A region, draw a **magnifying‑glass style inset** (zoomed box) placed near the bottom or side of the panel:
       - Show a zoomed‑in mini bar chart only for **A** (NaVILA‑A vs. SpikeVLA‑A) in that metric.
       - Maintain **the original units**:
         - Memory inset for A: values labeled in MB (NaVILA‑A: 1.20 MB, SpikeVLA‑A: 2.35 MB).  
         - Energy inset for A: values labeled in μJ (NaVILA‑A: 5.80 μJ, SpikeVLA‑A: 0.31 μJ).  
         - ACEs inset for A: values labeled in M (NaVILA‑A: 161.48 M, SpikeVLA‑A: 5.53 M).  
     - Draw connecting lines from the A section in the main axis to the inset, like a magnifying glass.

5. **Annotation emphasis**
   - Optionally annotate key relative improvements, e.g. near L bars:  
     - “SpikeVLA L uses ≈ 64% less memory than NaVILA L”  
     - “SpikeVLA L uses ≈ 68% less energy than NaVILA L”  
     - “SpikeVLA L uses ≈ 70% fewer ACEs than NaVILA L”  
   - Keep annotations minimal and clean, using small arrows or text without clutter.

---

### Right Panel: 6 pie charts (3 rows × 2 columns)

Goal: show the **internal distribution (V/L/A)** for each metric for NaVILA vs. SpikeVLA, and also show the **absolute scale difference** between NaVILA and SpikeVLA by scaling the pie chart size according to total Mem/Energy/ACEs. The Action (A) segments are extremely small and must be visually preserved with call‑outs and numerical ratios (percent / permille / ppm).

Layout:

- Arrange 6 pie charts in a grid: **3 rows × 2 columns**.  
- Column 1: **NaVILA**; Column 2: **SpikeVLA**.  
- Rows:
  - Row 1: Static Memory distribution (Mem).  
  - Row 2: Energy distribution.  
  - Row 3: ACEs distribution.  
- Add row labels on the left (Mem, Energy, ACEs) and column labels on top (NaVILA, SpikeVLA).

1. **Total values and pie size scaling**

Compute totals (per metric, per model):

- **NaVILA**
  - Total Memory ≈ 808.93 + 15316.05 + 1.20 ≈ 16126.18 MB  
  - Total Energy ≈ 22.70 + 118.55 + 5.80 μJ ≈ 141.25 J (5.80 μJ is negligible vs J but still kept in distribution)  
  - Total ACEs ≈ 631.52 T + 3298.69 T + 161.48 M  
    - Convert 161.48 M to 0.00016148 T  
    - Total ≈ 3921.83 T  

- **SpikeVLA**
  - Total Memory ≈ 809.88 + 5439.30 + 2.35 ≈ 6251.53 MB  
  - Total Energy ≈ 6.29 + 37.94 + 0.31 μJ ≈ 44.23 J  
  - Total ACEs ≈ 111.75 T + 997.86 T + 5.53 M  
    - Convert 5.53 M to 0.00000553 T  
    - Total ≈ 1109.61 T  

Pie size scaling rules:

- For each row (Mem, Energy, ACEs):
  - **NaVILA** pie (left) has a fixed reference radius (e.g., R = 1).  
  - **SpikeVLA** pie (right) has radius scaled by the ratio of SpikeVLA total to NaVILA total:
    - Memory: radius ≈ sqrt(6251.53 / 16126.18) ≈ 0.622 of NaVILA pie.  
    - Energy: radius ≈ sqrt(44.23 / 141.25) ≈ 0.56.  
    - ACEs: radius ≈ sqrt(1109.61 / 3921.83) ≈ 0.53.  
  - This produces visibly smaller pies for SpikeVLA in each row, reflecting lower total resource usage.

2. **Internal distribution within each pie (V/L/A fractions)**

Use three sectors per pie: V (Vision encoder), L (LLM), A (Action policy). Use a consistent color mapping across all pies:

- Vision encoder V: one color (e.g., dark blue).  
- LLM L: second color (e.g., light blue).  
- Action A: third color (e.g., gray or green).  

Proportions:

- **NaVILA – Memory**  
  - V: 808.93 / 16126.18  
  - L: 15316.05 / 16126.18  
  - A: 1.20 / 16126.18  

- **SpikeVLA – Memory**  
  - V: 809.88 / 6251.53  
  - L: 5439.30 / 6251.53  
  - A: 2.35 / 6251.53  

- **NaVILA – Energy**  
  - V: 22.70 / 141.25  
  - L: 118.55 / 141.25  
  - A: (5.80 μJ converted to J) / 141.25, but keep the sector visually preserved even though it is extremely tiny.

- **SpikeVLA – Energy**  
  - V: 6.29 / 44.23  
  - L: 37.94 / 44.23  
  - A: (0.31 μJ in J) / 44.23, again sector preserved visually.

- **NaVILA – ACEs**  
  - V: 631.52 / 3921.83  
  - L: 3298.69 / 3921.83  
  - A: 0.00016148 / 3921.83  

- **SpikeVLA – ACEs**  
  - V: 111.75 / 1109.61  
  - L: 997.86 / 1109.61  
  - A: 0.00000553 / 1109.61  

3. **Handling extremely small A segments**

- The A sector is extremely small for most pies but **must not disappear**.  
- Visually enforce a minimal visible angle for the A slice (a thin wedge) in each pie, even if it is larger than the true geometric proportion.  
- For each A segment, draw a **thin line from the tiny wedge to an external label (call‑out)**.  
- In the call‑out, report the **actual numeric fraction using appropriate units (percent / permille / ppm)**:
  - If A share > 1% use a percentage “x.xx%”.  
  - If between 0.1% and 1%, you may use “permille” ‰.  
  - If < 0.1%, use parts per ten thousand or parts per million “×10⁻⁴” or “×10⁻⁶”.  
- Example (you can compute more precise values in implementation, but conceptually):
  - NaVILA Memory A: roughly on the order of 0.01% or smaller → label like “A: ~0.01% of total Mem (1.20 MB)”.  
  - SpikeVLA Memory A: similarly small → label “A: ~0.04% of total Mem (2.35 MB)”.  
  - NaVILA Energy A: extremely tiny fraction of 141.25 J → label as “A: ~4×10⁻⁵ of total Energy (5.80 μJ)”.  
  - SpikeVLA Energy A: “A: ~7×10⁻⁶ of total Energy (0.31 μJ)”.  
  - NaVILA ACEs A: “A: ~4×10⁻⁸ of total ACEs (161.48 M)”.  
  - SpikeVLA ACEs A: “A: ~5×10⁻⁹ of total ACEs (5.53 M)”.  
- The exact numeric notation can be chosen for clarity, but every A sector must have:
  - A small visible wedge.  
  - A call‑out line.  
  - A numeric label reflecting its tiny ratio (percentage, permille, or scientific notation).

4. **Labels and legends for pies**

- For each pie chart, include a concise title inside or just above it, e.g.:
  - “Mem – NaVILA” / “Mem – SpikeVLA”  
  - “Energy – NaVILA” / “Energy – SpikeVLA”  
  - “ACEs – NaVILA” / “ACEs – SpikeVLA”  
- Include a small legend for V/L/A color coding, shared for all six pies (e.g., on the right side or bottom of the right panel).
- Clearly indicate unit conventions:
  - Memory labeled as MB.  
  - Energy labeled as J, with a note that microjoule values are included in the A sector.  
  - ACEs labeled with “T = 10¹², M = 10⁶”.

---

Global notes:

- Do **not** use logarithmic axes anywhere.  
- Maintain consistent color usage for:
  - **Model** (NaVILA vs. SpikeVLA) in bar charts.  
  - **Module** (V/L/A) in pie charts.  
- Ensure all texts are in **English**, with clear, publication‑grade typography.  
- The final figure should look like a main figure in an ICML paper: clean, high‑resolution, precise, and ready for LaTeX integration.
